Towards Radio Designs with Non-Linear Processing for Next Generation Mobile Systems

MIMO mobile systems, with a large number of antennas at the base-station side, enable the concurrent transmission of multiple, spatially separated information streams and, therefore, enable improved network throughput and connectivity both in uplink and downlink transmissions. Traditionally, to efficiently facilitate such MIMO transmissions, linear base-station processing is adopted, that translates the MIMO channel into several single-antenna channels. Still, while such approaches are relatively easy to implement, they can leave on the table a significant amount of unexploited MIMO capacity. Recently proposed non-linear base-station processing methods claim this unexplored capacity and promise a substantially increased network throughput. Still, to the best of the authors' knowledge, non-linear base-station processing methods not only have not yet been adopted by actual systems, but have not even been evaluated in a standard-compliant framework, involving of all the necessary algorithmic modules required by a practical system. This work, outlines our experience by trying to incorporate and evaluate the gains of non-linear base-station processing in a 3GPP standard environment. We discuss the several corresponding challenges and our adopted solutions, together with their corresponding limitations. We report gains that we have managed to verify, and we also discuss remaining challenges, missing algorithmic components and future research directions that would be required towards highly efficient, future mobile systems that can efficiently exploit the gains of non-linear, base-station processing.

==> sections/standard_limitations.tex <==
\subsection{Impact of SRS power control on non-linear}
\Gls{srs} power control is described in TS 38.213 (section 7.3). In 5G-NR transmit power for PUSCH and \gls{srs} is controlled separately using two independent (open and closed) power control loops.

This allows for the \gls{srs} to be transmitted with a constant power, whilst permitting PUSCH to be power controlled.

In case of LTE, until Rel-15 the SRS power control independent of PUSCH power control was possible only when the serving cell was not configured for PUCCH/PUSCH transmission which is the case for secondary TDD cells in TDD LTE CA scenarios [RP-162137]. In Rel-16, the concept of ''additional SRS'' was introduced. It permits independent control for the SRS and PUSCH transmit power. Similar to 5G-NR, this permits for the \gls{srs} to be transmitted with a constant power. The use of 

Based on the pathloss measurement and the adjustment state for the closed power control loop we can potentially estimate the channel magnitude difference between received signal power for multiple UEs. As SRS cannot be transmitted on some occasions, ... The approximation may differ depending on 


"SRS carrier switching (SRS-CS) was recently introduced in LTE Release 14 to assist the eNodeB (eNB) in obtaining the channel state information (CSI) of secondary TDD cells in TDD LTE CA scenarios. Prior to Release 14, only the primary cell benefits from SRS UE transmissions, and therefore downlink transmissions on secondary cells are done without prior knowledge of the CSI (Figure 8)."

\subsection{SRS capacity}

[RP182901] \gls{srs} capacity enhancements in release 16

"SRS has been proved to be a significant factor for DL MIMO performance, especially for massive MIMO in TDD. Although SRS has been enhanced in previous releases, e.g., SRS coverage enhancement in Release 14 FeMTC, Release 14 SRS carrier based switching, further improvement is still needed. Firstly, SRS coverage enhancement is typically implemented in special subframe, which restricts the number of supportable UEs that require SRS coverage enhancement. Introducing virtual cell ID is another way to increase SRS capacity through allowing different UEs to have different SRS sequences even occupying the same time-frequency resources. "



[TR36.897] SRS capacity enhancements (release 13/14). 

[R1-152983]"In LTE Rel-8, as UL SU-MIMO is not supported, at most 16 SRS with maximum SRS bandwidth can be multiplexed in each uplink sub-frame thanks to two transmission combs and eight usable cyclic shifts. While in Rel-10 LTE-A, due to SU-MIMO, each UE may be configured with multiple antennas, therefore the number of supportable UEs with SRS transmission in one subframe is decreased. For example, only four UEs would be supported in one uplink sub-frame when each of them is configured with four antennas and maximum SRS bandwidth, as four SRS resources are required for each UE. 

To provide additional SRS scheduling flexibility and potentially improve the SRS resource utilization, aperiodic SRS was introduced in Rel-10. However, since aperiodic SRS shares resources with periodic SRS, the total cell specific physical SRS resource is still the same as in Rel-8. As a result, it seems difficult to achieve timely on demand aperiodic SRS scheduling, considering the potential collision between aperiodic and periodic SRS and the signalling flexibility.

In Rel-11, to obtain reliable SRS-based channel estimates in UL CoMP, it is beneficial to coordinate SRS scheduling among multiple cells. Orthogonal SRS among multiple cells can be achieved by the coordination of orthogonal codes sequence, time and frequency resource. It means that one CoMP UE may occupy certain SRS resources of multiple cells. As a result, SRS resource will become much scarcer than that in Rel-10. Hence, SRS capacity enhancement is still desirable. 

In Rel-13, as more users will be scheduled by eNodeB under the deployment of FD-MIMO.  SRS would be used not only for UL channel state estimation but also for DL CSI estimation when channel reciprocity is applied.  Requirement on SRS capacity would become higher. The SRS shortage could be alleviated by some solutions, such as increasing the code sequence and comb, sounding based on non-precoded DMRS, or precoded SRS."

\subsection{Soft Input Soft Output}

Standard limitations? What is the impact of HARQ?

Interleaving, rate-matching and scrambling for the UL signal needs to be performed for each iteration. This should be added to [TS36.212] channel coding specification?

\subsection{PDCCH signaling}


%https://vbn.aau.dk/ws/files/249119871/KIP_Globecom_FlexTTI_Scheduling_FINAL_PID1185290.pdf <-- discusses PDCCH blocking

"The hashing function used to map Control Channel Elements (CCE) carrying DCI packets in the search space for each user may cause two PDCCH candidate sets to collide which leads to denial of allocation of control information for some users"

"The main problem in the search space allocation scheme in the LTE standard is that all the candidates are contiguous and the hashing function is only used to determine its starting point. This means that if the search spaces of 2 UEs collided in one of the candidates, it is highly probable that the next candidate of both UEs will collide as well, as shown in Fig 2 of LTE, and thus causes the low throughput problem stated earlier as one of the main problems of PDCCH.

Whereas in NR because of the scattering of the candidate at the NR-Search Space, there is less probability of the next candidate of both UEs will collide and get blocked."

\subsection{DMRS related bottlenecks}




\subsection{PUCCH signaling}

PUCCH in LTE and 5G-NR is the control channel used to transmit uplink control information (UCI) in the absence of uplink user data transmission over PUSCH channel. UCI carries different types of information, including HARQ ACKs/NACKs, Scheduling Requests (SR) and CSI (Channel State Information). The PUCCH design in both LTE and 5G-NR is flexible and allow for simultaneous transmission of UCI for multiple UEs at the expense of a higher control overhead.

LTE related

In case of LTE this does not seem to be a problem (pucch format 1b should be sufficient for a single layer MU-MIMO). Depending on the number of UEs in the cell, in order to prevent an excessive overhead in uplink, ...   

5G-NR related 
In case 5G-NR, PUCCH format 2,3 or 4 are required to be used in order to allow for transmission of sufficient number of ACKs in order to allow for TDD operation. The capacity of the PUCCH channel depends on a number of factors, including system bandwidth (or BWP), maximum allowed code rate, or slot UL/DL slot configuration. This translates to the maximum UCI size, and the number of UEs that can be 
